Mining Brain Networks using Multiple Side Views for Neurological Disorder Identification

Mining discriminative subgraph patterns from graph data has attracted great interest in recent years. It has a wide variety of applications in disease diagnosis, neuroimaging, etc. Most research on subgraph mining focuses on the graph representation alone. However, in many real-world applications, the side information is available along with the graph data. For example, for neurological disorder identification, in addition to the brain networks derived from neuroimaging data, hundreds of clinical, immunologic, serologic and cognitive measures may also be documented for each subject. These measures compose multiple side views encoding a tremendous amount of supplemental information for diagnostic purposes, yet are often ignored. In this paper, we study the problem of discriminative subgraph selection using multiple side views and propose a novel solution to find an optimal set of subgraph features for graph classification by exploring a plurality of side views. We derive a feature evaluation criterion, named gSide, to estimate the usefulness of subgraph patterns based upon side views. Then we develop a branch-and-bound algorithm, called gMSV, to efficiently search for optimal subgraph features by integrating the subgraph mining process and the procedure of discriminative feature selection. Empirical studies on graph classification tasks for neurological disorders using brain networks demonstrate that subgraph patterns selected by the multi-side-view guided subgraph selection approach can effectively boost graph classification performances and are relevant to disease diagnosis.

==> table_mainresults.tex <==
\begin{table*}[!ht]
\caption{Classification performance on the fMRI dataset with different number of features. The best performance of each method is in bold.}
\label{tab:result1}
\centering
\begin{tabular}{lccccccccccc}
\toprule%----------------------------
& \multicolumn{5}{c}{Accuracy} & \multicolumn{5}{c}{F1}\\
\cmidrule{2-6} \cmidrule{8-12}
Methods	&$k=60$ &$k=70$ &$k=80$ &$k=90$ &$k=100$ & &$k=60$ &$k=70$ &$k=80$ &$k=90$ &$k=100$ \\
\midrule %---------------------------
{\galgo}	&0.659 &0.687 &0.672 &0.672 &\textbf{0.701} & &0.657 &0.688 &0.682 &0.688 &\textbf{0.716} \\
{\gssc}		&0.529 &0.529 &0.530 &0.530 &\textbf{0.542} & &0.547 &0.547 &0.557 &0.557 &\textbf{0.566} \\
{\duga}	&0.558 &\textbf{0.600} &\textbf{0.600} &\textbf{0.600} &0.557 & &0.537 &\textbf{0.548} &0.533 &0.533 &0.452 \\
{\dugb}	&0.558 &\textbf{0.600} &\textbf{0.600} &\textbf{0.600} &0.557 & &0.537 &\textbf{0.548} &0.533 &0.533 &0.452 \\
{\dugc}	&0.571 &\textbf{0.572} &\textbf{0.572} &0.542 &0.556 & &\textbf{0.587} &0.586 &0.586 &0.556 &0.579 \\
{\dugd}	&\textbf{0.600} &\textbf{0.600} &0.556 &0.472 &0.528 & &0.579 &\textbf{0.579} &0.509 &0.433 &0.520 \\
{\topk}		&0.601 &\textbf{0.644} &0.586 &0.586 &0.601 & &0.650 &\textbf{0.692} &0.633 &0.633 &0.643 \\
\bottomrule%-------------------------
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\caption{Classification performance on the DTI dataset with different number of features. The best performance of each method is in bold.}
\label{tab:result2}
\centering
\begin{tabular}{lccccccccccc}
\toprule%----------------------------
& \multicolumn{5}{c}{Accuracy} & \multicolumn{5}{c}{F1}\\
\cmidrule{2-6} \cmidrule{8-12}
Methods	&$k=60$ &$k=70$ &$k=80$ &$k=90$ &$k=100$ & &$k=60$ &$k=70$ &$k=80$ &$k=90$ &$k=100$ \\
\midrule %---------------------------
{\galgo}	&0.606 &0.592 &0.645 &0.671 &\textbf{0.724} & &0.570 &0.551 &0.632 &0.679 &\textbf{0.704} \\
{\gssc}		&0.578 &0.578 &\textbf{0.593} &0.540 &0.553 & &0.566 &0.589 &\textbf{0.594} &0.531 &0.541 \\
{\duga}	&\textbf{0.567} &0.474 &0.527 &0.539 &0.513 & &\textbf{0.565} &0.436 &0.495 &0.518 &0.486 \\
{\dugb}	&0.592 &\textbf{0.605} &\textbf{0.605} &0.552 &0.553 & &0.651 &0.638 &\textbf{0.654} &0.594 &0.584 \\
{\dugc}	&\textbf{0.567} &0.541 &0.566 &0.553 &0.553 & &0.572 &0.580 &\textbf{0.602} &0.585 &0.574 \\
{\dugd}	&0.499 &0.527 &\textbf{0.553} &\textbf{0.553} &\textbf{0.553} & &0.557 &0.581 &\textbf{0.595} &\textbf{0.595} &\textbf{0.595} \\
{\topk}		&0.487 &\textbf{0.539} &0.487 &0.474 &\textbf{0.539} & &0.517 &0.596 &0.541 &0.543 &\textbf{0.615} \\
\bottomrule%-------------------------
\end{tabular}
\end{table*}
